DistDD: Distributed Data Distillation Aggregation through Gradient Matching

In this paper, we introduce DistDD, a novel approach within the federated learning framework that reduces the need for repetitive communication by distilling data directly on clients' devices. Unlike traditional federated learning that requires iterative model updates across nodes, DistDD facilitates a one-time distillation process that extracts a global distilled dataset, maintaining the privacy standards of federated learning while significantly cutting down communication costs. By leveraging the DistDD's distilled dataset, the developers of the FL can achieve just-in-time parameter tuning and neural architecture search over FL without repeating the whole FL process multiple times. We provide a detailed convergence proof of the DistDD algorithm, reinforcing its mathematical stability and reliability for practical applications. Our experiments demonstrate the effectiveness and robustness of DistDD, particularly in non-i.i.d. and mislabeled data scenarios, showcasing its potential to handle complex real-world data challenges distinctively from conventional federated learning methods. We also evaluate DistDD's application in the use case and prove its effectiveness and communication-savings in the NAS use case.

==> sec/12_rebuttal.tex <==
\newpage
\onecolumn

\newcommand{\question}[1]{\textcolor{blue}{\vspace*{0.05in}\noindent\textbf{#1}}}
\newcommand{\answer}[1]{\textcolor{green}{\vspace*{0.05in}\noindent\textbf{#1}}}

\section{Rebuttal}

Thanks for your careful and valuable comments. We will explain your concerns point by point.

\subsection{Reviewer NuAK}

\question{Q1}: The motivation of data distillation for enabling hyper-parameter tuning is not emphasized enough in the introduction. Best exposure comes from the beginning of Section 3.

\answer{A1}: Thanks for the mention. We added the 2 use cases in the introduction to emphasize the use of \sysname.

\sssec{Use Case A (Multiple parameter tuning times)}: Unlike the debugging of a typical FL process which requires multiple communication iterations, our proposed method, \sysname\ distillates the data from distributed clients rather than just directly training a single classifier model. By acquiring this distilled dataset, FL servers can iteratively train the global model on the distilled dataset locally without iteratively debugging the parameters of FL, thus avoiding heavy communication costs.

\sssec{Use Case B (NAS over FL)}: Furthermore, the distilled dataset of \sysname\ can also be utilized for continuous learning and Neural Architecture Search(NAS). For instance, the FL server wants to design a neural network that has the best performance on the given FL tasks. If the server directly repeats multiple FL processes to execute the NAS, the time cost would be rather high. However, if the server just acquired the distilled dataset first, then doing the NAS using the dataset. Thus the cost of NAS can be saved.

\question{Q2}: Table 1 is misleading, and I think it should showcase the absolute test accruacies for all the methods instead of differences; the reader should infer the reason for performance drop (whether distillation or distributed nature of data) themselves.

\answer{A2}: Thanks for the point. We added the absolute accuracy to Table 1. Our initial attempt is to inform readers of the difference between centralized training (centralized GM) and decentralized FL (decentralized GM). This is used to indicate how decentralized affects DistDD's accuracy. We make the comparison since data distillation can not overcome the original algorithm. We will restore it back to the absolute accuracy version,

\question{Q3}: We observe that network trained on distilled data performs notably worse than FedAvg, I would suggest doing a case study for hyper-parameter tuning, e.g. let us say we want to tune the learning rate in distilled dataset, will it give the same results as if we tune it during FedAvg? This would be a realistic use case for your method.

\answer{A3}: Thanks for the mention. We provide two use cases following. According to the two use cases we mentioned above, making the distilled dataset have the same performance as the original dataset over FedAvg is unrealistic. However, you can complete the multiple tuning processes or multiple NAS processes to find the best parameter and best neural network architecture using the distilled dataset at first. Then, using the parameter and the network, you can train the FL process on it. This is our main contribution to the FL community. We will further provide a use case evaluation on parameter tuning and NAS in the evaluation section.

\question{Q4}: The theoretical contribution are straightforward and although they are mentioned in introduction and contributions; they are only to be found in appendix.

\answer{A4}: Thanks for the point. We will provide the brief proof statement in the main text.

\question{Q5}: There are many typos in the proofs, and the way the equations are formatted is not reader friendly.

\answer{A5}: Thanks for the mention. We will fix the typos in the proofs and make the equations more readable.


\subsection{Reviewer HsSq}

\question{Q1}: The proposed approach does not show clear advantage than FedAvg. From Table 1 and Figure 5, DistDD is even worse than FedAvg in many cases, especially in the non-IID cases. The paper mentioned communication costs as a motivation. But comparing FedAvg and DistDD, I did not find any additional hyper-parameter tuning for FedAvg. The paper should clearly present the communication costs if DistDD can indeed save more communication costs.

\answer{A1}: To be noted, as a data distillation approach, \sysname\ does not aim to achieve better model performance than FedAvg. We added the 2 use cases in the introduction (\ref{sec:intro}) to emphasize how can we use \sysname\ in FL.

\sssec{Use Case A (Multiple parameter tuning times)}: Unlike the debugging of a typical FL process which requires multiple communication iterations, our proposed method, \sysname\ distillates the data from distributed clients rather than just directly training a single classifier model. By acquiring this distilled dataset, FL servers can iteratively train the global model on the distilled dataset locally without iteratively debugging the parameters of FL, thus avoiding heavy communication costs.

\sssec{Use Case B (NAS over FL)}: Furthermore, the distilled dataset of \sysname\ can also be utilized for continuous learning and Neural Architecture Search(NAS). For instance, the FL server wants to design a neural network that has the best performance on the given FL tasks. If the server directly repeats multiple FL processes to execute the NAS, the time cost would be rather high. However, if the server just acquired the distilled dataset first, then doing the NAS using the dataset. Thus the cost of NAS can be saved.

\par And for the two cases, we plan to add the evaluation regarding how the accuracy and communication differs of the two cases between FedAvg and \sysname.

\question{Q2}: The presentation could be further improved. It’d be better if the authors put the theorems in the main paper while maintaining proof in Appendix. Currently, the convergence analysis is even not clearly mentioned in the main paper.

\answer{A2}: Thanks for the mention, we will provide the brief proof statement in the main text.

\question{Q3}: When applying DP, it’d be better to compare with DP-FedAvg too.

\answer{A3}: Thanks for the mention, we will add the comparison of DP-FedAvg.

\question{Q4}: Why would people choose DistDD if it is even worse than FedAvg? What are the benefits of DistDD compared with FedAvg especially in the non-IID data setting?

\answer{A4}: To be noted, as a data distillation approach, \sysname\ does not aim to achieve better model performance than FedAvg. We added the 2 use cases above (it will be added to the introduction section) to emphasize how can we use \sysname\ in FL. The distilled dataset is to provide efficient parameter tuning and NAS for FL, then you can use the tuned parameter and searched network architecture to complete the FL process.

\question{Q5}: How is the data partitioned among clients? The paper only mention dir without detailed introduction.

\answer{A5}: Thanks for mention. We will add the data partition statement.

\sssec{Data distribution.} In this experiment, we used the Dirichlet distribution to guide the data segmentation process. The Dirichlet distribution is a multinomial distribution that is often used to represent the probability distribution of multiple categories and is very suitable for simulating the distribution of different categories in a data set. The concentration parameter $\alpha$ of the Dirichlet distribution (we noted as $dir$) is used to guide the non-iid degree of the distribution.


\subsection{Reviewer PHtj}

\question{Q1}: Could the authors make more comparisons and indicate the contribution?

\answer{A3}: Thanks for the mention. 

\par For your question: ``The authors claimed the contribution of "computation" in Abstract and Section 5. However, except for one mention in Line 215, there is no analysis or experiment to verify the contribution.'', we added the comparison of multiple iterations of parameter tuning time cost between FedAvg and \sysname, which indicated \sysname's ability to save time cost (in computation and communication).

\par For your question: ``The idea of "running the federated learning framework once" in Abstract is not new. The key contribution in Section 2.2 of the new scene for dataset distillation is not new in federated learning. For example, "Federated Learning via Decentralized Dataset Distillation in Resource-Constrained Edge Environments" (IJCNN, 2023), "Communication-efficient federated learning via knowledge distillation" (Neural Communications, 2022), "Ensemble Distillation for Robust Model Fusion in Federated Learning", (NeurIPS, 2020)'', 

\par Our \sysname\ is not aimed to simply introduce DD into FL to enhance accuracy, but explore how DD can be utilized in a new paradigm for FL. \sysname\ aims to provide data distillation for more efficient parameter tuning and NAS, etc.

\par For your question: ``After reading Section 3 in detail, unfortunately, I found nothing new in the contribution of "gradient matching," as mentioned in the title.'', gradient matching is not our original work, our work aims at how to apply gradient matching into FL scene to provide sufficient hyper-parameter tuning.

\par For your question: ``The comparison in Section 4 is mostly with "FedAvg", which is not very recent. There is a branch of improved works (>10K citations now) following FedAvG, but none of them was chosen to be compared.'', we will add the comparison with FedProx in Table. \ref{tab:perf} later.

\question{Q2}: Could the authors add privacy analysis specific to the proposed idea?

\answer{A2}: Thanks for the mention, we will provide privacy analysis later.

\question{Q3}: Could the authors analyze the experimental results with a deeper understanding?

\answer{A3}: Thanks for the mention. We will add more deeper analysis soon.

==> sec/6-1-proof-re_f.tex <==
\section{\rebuttal{Convergence Proof}}\label{sec:proof}

\par \rebuttal{We formulate the proof of our \sysname\ as two steps: First we prove the convergence of our FL process. Then we prove the convergence of the gradient matching process by proving that the synthetic dataset can be very close to the original dataset. The detailed proof process is stated in Sec. \ref{sec:appendix:proof}.}

\par \rebuttal{We first makes a traditional federated learning convergence proof process, then we proved that the distilled dataset is almost same with the original dataset:}

\begin{equation}
    \sum_{t=0}^{T-1}\left\|\nabla D\left(S_{t}\right)\right\|^{2} \leq \frac{D\left(S_{0}\right)-D^{*}}{\eta_{\mathcal{S}}-\frac{L \eta_{\mathcal{S}}^{2}}{2}}
\end{equation}

==> sec/7-checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textcolor{red}{yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textcolor{red}{yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \textcolor{red}{yes}
    \item Does this paper make theoretical contributions? \textcolor{red}{yes}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. \textcolor{red}{yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \textcolor{red}{yes}
    \item Proofs of all novel claims are included. \textcolor{red}{yes}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textcolor{red}{yes}
    \item Appropriate citations to theoretical tools used are given. \textcolor{red}{yes}
    \item All theoretical claims are demonstrated empirically to hold. \textcolor{red}{yes}
    \item All experimental code used to eliminate or disprove claims is included. \textcolor{red}{yes}
    \item Does this paper rely on one or more datasets? \textcolor{red}{yes/no}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets \textcolor{red}{yes}
    \item All novel datasets introduced in this paper are included in a data appendix. \textcolor{red}{NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textcolor{red}{NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textcolor{red}{yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textcolor{red}{yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textcolor{red}{NA}
    \item Does this paper include computational experiments? \textcolor{red}{no}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textcolor{red}{yes}.
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textcolor{red}{yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textcolor{red}{yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textcolor{red}{yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textcolor{red}{NA}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textcolor{red}{yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textcolor{red}{yes}
    \item This paper states the number of algorithm runs used to compute each reported result. \textcolor{red}{yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textcolor{red}{yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textcolor{red}{yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textcolor{red}{yes}
\end{itemize}

==> sec/archive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|lll|lll|lll|}
\hline
Datasets & \multicolumn{3}{c|}{MNIST} & \multicolumn{3}{c|}{FashionMNIST} & \multicolumn{3}{c|}{CIFAR} \\ \hline\hline
NonIID & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 \\ \hline
Whole Dataset & \multicolumn{3}{c|}{99.3} & \multicolumn{3}{c|}{93.6} & \multicolumn{3}{c|}{87.2} \\ \hline
Gradient Matching(IPC=10) & \multicolumn{3}{c|}{96.3} & \multicolumn{3}{c|}{86.2} & \multicolumn{3}{c|}{52.3} \\ \hline
FedAvg & \multicolumn{1}{l|}{98.7} & \multicolumn{1}{l|}{94.3} & 85.1 & \multicolumn{1}{l|}{92.5} & \multicolumn{1}{l|}{86.3} & 74.3 & \multicolumn{1}{l|}{86.3} & \multicolumn{1}{l|}{75.3} & 65.9 \\ \hline
DistDD(IPC=10) & \multicolumn{1}{l|}{94.1} & \multicolumn{1}{l|}{90.3} & 82.3 & \multicolumn{1}{l|}{82.1} & \multicolumn{1}{l|}{75.3} & 67.6 & \multicolumn{1}{l|}{51.3} & \multicolumn{1}{l|}{47.4} & 41.5 \\ \hline
DistDD(IPC=50) & 
\multicolumn{1}{l|}{95.6} & \multicolumn{1}{l|}{92.8} & 83.1 & 
\multicolumn{1}{l|}{84.7} & \multicolumn{1}{l|}{82.5} & 69.3 & 
\multicolumn{1}{l|}{75.2} & \multicolumn{1}{l|}{62.4} & 51.5 \\ \hline

DistDD(IPC=100) & 
\multicolumn{1}{l|}{96.9} & \multicolumn{1}{l|}{93.2} & 83.9 & 
\multicolumn{1}{l|}{90.1} & \multicolumn{1}{l|}{84.3} & 72.5 & 
\multicolumn{1}{l|}{78.2} & \multicolumn{1}{l|}{69.2} & 57.3 \\ \hline\hline
\end{tabular}%
}
\caption{The performance comparison to the whole dataset (centralized training using the whole dataset), gradient matching (centralized gradient matching using the whole dataset), FedAvg(federated learning using FedAvg algorithm), and DistDD. For FedAvg and DistDD, we set the client number to 50. it seems this table will be easily questioned: our results do not outperform Fedavg or gradient matching, then reviewers can easily jump over the logic reasoning and ask for evidence that our method is useful. maybe we can show how much standard FedAvg and approach whole datasets, and use that to compare how much distDD can approach gradient matching, and same for the federated part.
Sorry, I do not get your point. You mean we can compare A:[whole dataset - Federated Learning] with B:[whole dataset gradient matching - DistDD]?

}
\label{tab:perf}
\end{table*}

\begin{figure}[!htp]
  \centering
    \subfloat[MNIST]{\includegraphics[width=0.165\textwidth]{figs/vis_DC_MNIST_ConvNet_10ipc_exp0_iter500.png}}
    \subfloat[FashionMNIST]{\includegraphics[width=0.165\textwidth]{figs/vis_DC_FashionMNIST_ConvNet_10ipc_exp0_iter500.png}}
    \subfloat[CIFAR]{\includegraphics[width=0.165\textwidth]{figs/vis_DC_CIFAR10_ConvNet_10ipc_exp0_iter500.png}}
  \\
  \caption{Generated Images of \sysname\ under IID data distribution.}
  \label{fig_exp_bs}
  \vspace{0.2in}
\end{figure}

\begin{table*}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2cm}|lll|lll|lll|}
\hline

Datasets & \multicolumn{3}{c|}{MNIST} & \multicolumn{3}{c|}{FashionMNIST} & \multicolumn{3}{c|}{CIFAR} \\ \hline\hline

NonIID & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 & \multicolumn{1}{l|}{dir=1(IID)} & \multicolumn{1}{l|}{dir=0.5} & dir=0.1 \\ \hline

Whole Dataset & \multicolumn{3}{c|}{99.3} & \multicolumn{3}{c|}{93.6} & \multicolumn{3}{c|}{87.2} \\ \hline

%Gradient Matching(IPC=10) & \multicolumn{3}{c|}{96.3} & \multicolumn{3}{c|}{86.2} & \multicolumn{3}{c|}{52.3} \\ \hline

GM (IPC=100) & 
\multicolumn{3}{c|}{97.2} & \multicolumn{3}{c|}{91.1} & \multicolumn{3}{c|}{80.7} \\ \hline

\pr{FedAvg} & 
\multicolumn{1}{l|}{-0.5} & \multicolumn{1}{l|}{-5.0} & -6.8 & 
\multicolumn{1}{l|}{-1.1} & \multicolumn{1}{l|}{-7.3} & -19.3 & 
\multicolumn{1}{l|}{-0.9} & \multicolumn{1}{l|}{-11.9} & -21.3 \\ \hline

\pr{DistDD (IPC=10)} & 
\multicolumn{1}{l|}{-3.1} & \multicolumn{1}{l|}{-6.9} & -14.9 & 
\multicolumn{1}{l|}{-9.0} & \multicolumn{1}{l|}{-15.8} & -23.5 & 
\multicolumn{1}{l|}{-29.4} & \multicolumn{1}{l|}{-33.3} & -39.2 \\ \hline

\pr{DistDD (IPC=50)} & 
\multicolumn{1}{l|}{-1.6} & \multicolumn{1}{l|}{-4.4} & -14.1 & 
\multicolumn{1}{l|}{-6.4} & \multicolumn{1}{l|}{-8.6} & -21.8 & 
\multicolumn{1}{l|}{-5.5} & \multicolumn{1}{l|}{-18.3} & -29.2 \\ \hline

\pr{DistDD (IPC=100)} & 
\multicolumn{1}{l|}{-0.3} & \multicolumn{1}{l|}{-4.0} & -13.2 & 
\multicolumn{1}{l|}{-1.0} & \multicolumn{1}{l|}{-6.8} & -18.6 & 
\multicolumn{1}{l|}{-2.5} & \multicolumn{1}{l|}{-11.5} & -23.4 \\ \hline\hline
\end{tabular}%
%}
\caption{The performance comparison to the whole dataset (centralized training using the whole dataset), GM (centralized gradient matching using the whole dataset), FedAvg(federated learning using FedAvg algorithm), and DistDD. For FedAvg and DistDD, we set the client number to 50. The FedAvg's accuracy value is compared with the whole dataset training and recorded in the table. The \sysname's accuracy is compared with the gradient matching's accuracy (IPC=100) and recorded in the table. The comparison between (FedAvg-Whole dataset) and (\sysname\ - GM) indicates that \sysname's performance aligns with FedAvg on the distributed pattern.}
\label{tab:perf}
\end{table*}

==> sec/meet_summary.tex <==
# Internal Review

- Place mislabeling and non-iid in a more important place. (done)
- Archive the ablation study (done)

- Try to make fedavg better than local (doing)
- Explain the solution of mislabeling and non-iid clearly (doing)
- State the DP you used in the experiment (doing)
- The updated gradient changes to the real images' gradient rather than synthetic images' (exp running)

- The difference between each local data distillation, and send to the server (ablation study, in the node number)


- the figure too large, adjust to single column
- modify the abstract
- different
- delete KD literature
